Strassen's Algorithm for Tensor Contraction

Tensor contraction (TC) is an important computational kernel widely used in numerous applications. It is a multi-dimensional generalization of matrix multiplication (GEMM). While Strassen's algorithm for GEMM is well studied in theory and practice, extending it to accelerate TC has not been previously pursued. Thus, we believe this to be the first paper to demonstrate how one can in practice speed up tensor contraction with Strassen's algorithm. By adopting a Block-Scatter-Matrix format, a novel matrix-centric tensor layout, we can conceptually view TC as GEMM for a general stride storage, with an implicit tensor-to-matrix transformation. This insight enables us to tailor a recent state-of-the-art implementation of Strassen's algorithm to TC, avoiding explicit transpositions (permutations) and extra workspace, and reducing the overhead of memory movement that is incurred. Performance benefits are demonstrated with a performance model as well as in practice on modern single core, multicore, and distributed memory parallel architectures, achieving up to 1.3x speedup. The resulting implementations can serve as a drop-in replacement for various applications with significant speedup.

==> ae.tex <==
\appendix
\section{Artifact Description: [{ Strassen's Algorithm for Tensor Contraction}]}

\subsection{Abstract}
The artifact contains all components of the implementations and benchmarks
of Strassen's algorithm for tensor contraction
submitted to SC 17.

\subsection{Description}


\subsubsection{Check-list (artifact meta information)}

{\small
%\begin{itemize}
\begin{itemize}[leftmargin=*]
  \item {\bf Algorithm: } \ABCstrassen{}, \ABXstrassen{}, \XXXstrassen{}, and \tblis{} tensor contraction.
  \item {\bf Program: } {\tt C99}, {\tt C++11}, {\tt MPI}, {\tt AVX inline assembly}
  \item {\bf Compilation: }
  MPI C/C++ compiler (C99/C++11 capable); we use icc/icpc version 15.0.3 with the gcc 4.9.3 Standard Template Library for single node experiment; mpicc/mpicxx in mvapich2/2.1 for distributed memory experiment.
  \item {\bf Data set: }
  Sythetic dataset and Tensor Contraction Benchmark.
  %\item {\bf Run-time environment: }
  %Specified in the execution scripts, e.g. {\tt OMP\_NUM\_THREADS}, {\tt KMP\_AFFINITY}, etc. 
  \item {\bf Hardware: }
  Maverick supercomputer at TACC.
%\footnote{https://portal.tacc.utexas.edu/user-guides/maverick}
  \item {\bf Output: }
  \emph{Effective} GFLOPS performance, as shown \mycircle{1} in \figref{tab:perfmodel}. 
  \item {\bf Experiment workflow: }
  Decompress the source code, configure and compile the code, check the dataset and environment, and execute the code.
  \item {\bf Publicly available?: }
  Omitted due to double blind review policy.
\end{itemize}
}

\subsubsection{How software can be obtained (if available)}
Due to the double blind review policy, the source code can be obtained
in anonymous Google Drive folder:
{\color{blue}{\href{https://goo.gl/qW4IY6}{https://goo.gl/qW4IY6}}}

\subsubsection{Hardware dependencies}
x86-64 processor that supports {\tt AVX} instructions.

\subsubsection{Software dependencies}
Linux or macOS/OS X,
{\tt autotools},
Intel icc/icpc compiler 15 or later and compatible GCC 4.9 or later,
mvapich2/2.1 for {\tt MPI},
{\tt OpenMP} environment, SLURM queuing system (for distributed experiments---the
details of the TACC Maverick job queues are assumed in the provided scripts).

\subsubsection{Datasets}
Synthetic data and some representative use cases from 
Tensor Contraction Benchmark \cite{TCB}.

\subsection{Installation}

Follow the build instructions in {\tt README.md}, found in the source code top folder
after extracting the
{\tt tblis-strassen.tar.gz} from the
{\color{blue}{\href{https://goo.gl/qW4IY6}{\tt URL}}}
above.

\subsection{Experiment workflow}

\begin{itemize}[leftmargin=*]
\item Download {\tt tblis-strassen.tar.gz} from the
{\color{blue}{\href{https://goo.gl/qW4IY6}{\tt URL}}}
above.

\item Compile the source code:
Replace 
{\tt \$INSTALL\_PATH} with the installation path the user wants to specify.

\begin{verbatim}
$ tar -zxvf tblis-strassen.tar.gz
$ cd tblis-strassen
$ autoreconf -i
$ ./configure --prefix=$INSTALL_PATH \
    --disable-shared --enable-config=sandybridge
$ make && make install
\end{verbatim}

\item Set up environment variables:
Replace {\tt \$core\_num} with the number of cores the user wants to run.

\begin{verbatim}
$ export OMP_NUM_THREADS=$core_num
$ export KMP_AFFINITY=compact
\end{verbatim}

Note: if hyper-threading is enabled, the following alternative must be used:

\begin{verbatim}
$ export KMP_AFFINITY=compact,1
\end{verbatim}

\item Single node experiment (synthetic tensor contractions):
Replace {\tt \$NIm} with $\NIm{}$, {\tt \$NJn} with $\NJn{}$,
{\tt \$NPk} with $\NPk{}$, {\tt \$niter} with the iterations the user wants to run,
{\tt \$L} with number of levels of \strassen{} to employ ($L=0$ will invoke regular \tblis{} TC routine),
and {\tt \$IMPL} with the implementations the user wants to test.
{\tt \$IMPL} has the following options,
[
$1$: \ABCstrassen{},
$2$: \ABXstrassen{},
$3$: \XXXstrassen{}
].

\begin{verbatim}
$ cd bin
$ ./test_strassen -m $NIm -n $NJn -k $NPk \
    -niter $niter -level $L -impl $IMPL
\end{verbatim}

%$ cd bin
%\item Run the code

We have prepared the testing scripts in {\tt bin} folder 
so the user can run it directly to reproduce the experiments in this paper
(e.g. {\tt square\_run\_1core.sh} ).

\item Single node experiment (real-world benchmark):

\begin{verbatim}
$ cd bin
$ ./test_strassen -file $benchmark_filename
\end{verbatim}

We have prepared the benchmark from \cite{TCB} as {\tt tcb.txt}
and the test scripts (e.g. {\tt tcb\_run\_1core.sh}) to make it easier
for the user to reproduce the result presented in this paper.

\item Single node experiment (shape-dependence experiment):

\begin{verbatim}
$ cd bin
$ ./test_strassen -file $shape_filename
\end{verbatim}

We have prepared the test cases we use as {\tt shape.txt}
and the test scripts (e.g. {\tt shape\_run\_1core.sh}) to make it easier
for the user to reproduce the result presented in this paper.

\item Distributed memory experiment:
Replace 
{\tt \$P} with the edge length of the $ P \times P $ mesh the user wants to test on.

\begin{verbatim}
$ cd dist
$ make
$ sbatch ./submit_${P}x${P}.sh
\end{verbatim}

\end{itemize}

\subsection{Evaluation and expected result}

The output will include the following components:
\begin{itemize}
\item Input problem size.
\item Running time (in seconds).
\item Total GFLOPS (floating point operation number).
\item \emph{Effective} GFLOPS (\mycircle{1} in \figref{tab:perfmodel}). 
\item Accuracy ($ \frac{ \| \T{T} - \T{T}_{ref} \|_2  }{ \| \T{T}_{ref} \|_2 } $ ).
\end{itemize}

The user can compare the relative \emph{Effective} GFLOPS for different implementations.
The trend should match the performance curves shown in this paper.
Since the machines may be different from ours, the absolute GFLOPS could be different.

\subsection{Experiment customization}

The format information for the user specified benchmark can be found in {\tt README.md}.
For instance, to evaluate the example
$ \T{C}_{a,b,c} +\!\!= \T{A}_{d,c,a} \cdot \T{B}_{d,b} $
in \figref{fig:stra_tensor},
the user can specify the following input:
%in the benchmark file:
\begin{verbatim}
    abc dca db & a:4;b:8;c:2;d:8;
\end{verbatim}

%\subsection{Notes}
%None.




==> figures/benchmark/preamble.tex <==
\usepackage{etex}

%\documentclass{sigplanconf}[10pt]
%\documentclass{sig-alternate}
%\documentclass{acm_proc_article-sp}
%\setlength{\textheight}{8.75in}
%\setlength{\textwidth}{6.5in}
%\setlength{\oddsidemargin}{0in}
%\setlength{\evensidemargin}{0in}
%\setlength{\topmargin}{-0.5in}

%\usepackage{amsmath}
\usepackage{comment}
\usepackage{tikz}
\usetikzlibrary{matrix,arrows,decorations.pathmorphing,patterns,positioning}
\usepackage{amssymb}
\usepackage{ifthen}
\usepackage{color}
\usepackage{colortbl}
\usepackage{rotating}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{url}
\usepackage{arydshln}

%\usepackage{pgfplots}
\usepackage{pgfplots}
%\pgfplotsset{compat=1.5}
%\pgfplotsset{compat=1.8}
%\usepgfplotslibrary{colorbrewer}

%\pgfplotsset{width=7cm,compat=1.13}

\usetikzlibrary{external}
\tikzexternalize[prefix=tikz/]

\usepackage{wrapfig}
%\usepackage{subfigure}
%\usepackage{subcaption}
\usepackage[font=small]{subcaption}
%\usepackage{caption}
%\usepackage[margin=0pt,labelsep=space,font=scriptsize,labelfont=bf,textfont=it,belowskip=-8pt,aboveskip=5pt]{caption}
%\usepackage[labelsep=space,font=small,aboveskip=5pt]{caption}
%\usepackage[font=small,labelfont=bf,textfont=normal,aboveskip=5pt]{caption}
\usepackage[font=small,labelfont=bf,textfont=it,aboveskip=5pt]{caption}
\usepackage{array}
\usepackage{framed}

\usepackage{balance}

\usepackage{epsfig}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
%\usepackage{algorithmicx}
%\usepackage{amsthm}

\usepackage{algorithmic}

%\usepackage[section]{algorithm}
\usepackage{algorithm}

\usepackage[normalem]{ulem}

%\usepackage{program}
\usepackage{ifthen}
\usepackage{boxedminipage}
\usepackage{fancyvrb}

\usepackage{soul}
\usepackage{graphicx}
\usepackage{graphics}
\usepackage{moreverb}
\usepackage{rotating}
\usepackage{enumerate}

\usepackage{enumitem}

\usepackage{tabularx,booktabs}

\usetikzlibrary{arrows}

%\usepackage{flushend}
\usepackage{xspace}

\usepackage{stmaryrd}



%\usepackage[absolute,showboxes]{textpos}
\usepackage[absolute]{textpos}
%set unit to be pagewidth and height, and increase inner margin of box
\setlength{\TPHorizModule}{\paperwidth}\setlength{\TPVertModule}{\paperheight}
\TPMargin{5pt}

\usepackage{listings}
\usepackage{xcolor}
\usepackage{fancyvrb}
\fvset{tabsize=2}
\definecolor{mygreen}{rgb}{0,0.6,0}
\lstset{ %
language=C,                % choose the language of the code
basicstyle=\footnotesize,       % the size of the fonts that are used for the code
commentstyle=\color{mygreen},
keywordstyle=\color{blue},
%numbers=left,                   % where to put the line-numbers
%numberstyle=\footnotesize,      % the size of the fonts that are used for the line-numbers
%stepnumber=1,                   % the step between two line-numbers. If it is 1 each line will be numbered
%numbersep=5pt,                  % how far the line-numbers are from the code
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
frame=single,           % adds a frame around the code
tabsize=1,          % sets default tabsize to 2 spaces
columns=fixed,
captionpos=b,           % sets the caption-position to bottom
breaklines=true,        % sets automatic line breaking
breakatwhitespace=true,    % sets if automatic breaks should only happen at whitespace
escapeinside={\%*}{*)}          % if you want to add a comment within your code
}            

%\pgfplotsset{every axis/.append style={
%        scaled y ticks = false, 
%        scaled x ticks = false, 
%        y tick label style={/pgf/number format/.cd, fixed, fixed zerofill,
%                            int detect,1000 sep={\;},precision=3},
%        x tick label style={/pgf/number format/.cd, fixed, fixed zerofill,
%                            int detect, 1000 sep={},precision=3}
%    }
%}

\special{papersize=8.5in,11in}
\setlength{\pdfpageheight}{\paperheight}
\setlength{\pdfpagewidth}{\paperwidth}

%\conferenceinfo{CONF 'yy}{Month d--d, 20yy, City, ST, Country} 
%\copyrightyear{20yy} 
%\copyrightdata{978-1-nnnn-nnnn-n/yy/mm} 
%\doi{nnnnnnn.nnnnnnn}

% Uncomment one of the following two, if you are not going for the 
% traditional copyright transfer agreement.

%\exclusivelicense                % ACM gets exclusive license to publish, 
                                  % you retain copyright

%\permissiontopublish             % ACM gets nonexclusive license to publish
                                  % (paid open-access papers, 
                                  % short abstracts)

%\titlebanner{banner above paper title}        % These are ignored unless
%\preprintfooter{short description of paper}   % 'preprint' option specified.


%\usepackage{lmodern}

\usepackage{afterpage}

%\usepackage{mathrsfs}
%% For \mathscr
\usepackage[mathscr]{eucal}

%bold math
\usepackage{bm}

\pgfplotscreateplotcyclelist{mycolorlist}{%
blue,every mark/.append style={fill=blue!80!black},mark=*\\%
red,every mark/.append style={fill=red!80!black},mark=square*\\%
brown!60!black,every mark/.append style={fill=brown!80!black},mark=otimes*\\%
black,mark=star\\%
blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
brown!60!black,densely dashed,every mark/.append style={
solid,fill=brown!80!black},mark=square*\\%
black,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,densely dashed,mark=star,every mark/.append style=solid\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*\\%
}



\definecolor{colorbrewer1}{RGB}{228,26,28}
\definecolor{colorbrewer2}{RGB}{55,126,184}
\definecolor{colorbrewer3}{RGB}{77,175,74}
\definecolor{colorbrewer4}{RGB}{152,78,163}
\definecolor{colorbrewer5}{RGB}{255,127,0}
%\definecolor{colorbrewer6}{RGB}{255,255,51}
\definecolor{colorbrewer7}{RGB}{166,86,40}
\definecolor{colorbrewer8}{RGB}{247,129,191}
\definecolor{colorbrewer9}{RGB}{153,153,153}

\definecolor{darkgreen}{rgb}{0,0.5,0}

\newcommand{\cblue}[1]{\textcolor{blue}{#1}}
\newcommand{\cgreen}[1]{\textcolor{darkgreen}{#1}}
\newcommand{\cpurple}[1]{\textcolor{purple}{#1}}
\newcommand{\cred}[1]{\textcolor{red}{#1}}

\definecolor{darkred}{rgb}{0.44,0,0}
\definecolor{darkgreen}{rgb}{0,0.44,0}
\definecolor{darkblue}{rgb}{0,0,0.44}
\definecolor{enrique}{rgb}{0,0,0}

\pgfplotscreateplotcyclelist{jianyu2color}{
	colorbrewer1, mark=*,\\
	colorbrewer2, mark=square*,\\
	colorbrewer3, mark=triangle*,\\
	colorbrewer4, mark=x,\\
	colorbrewer5, mark=*,\\
	%colorbrewer6, mark=square*, \\
	colorbrewer7, mark=triangle*,\\
	colorbrewer8, mark=+,\\
}

\pgfplotscreateplotcyclelist{jianyu0color}{%
thick,colorbrewer1,every mark/.append style={fill=colorbrewer1},mark=triangle*,only marks\\%
thick,orange,every mark/.append style={fill=orange},mark=square*,only marks\\%
thick, lime!80!black,every mark/.append style={fill=lime!80!black},mark=pentagon*,only marks\\%
%thick,red!70!white,mark=pentagon*,only marks\\%
thick,blue,every mark/.append style={fill=blue!80!black},mark=triangle*,only marks\\%
thick,cyan,every mark/.append style={fill=cyan},mark=square*,only marks\\%
thick,darkgreen,mark=pentagon*,only marks\\%
thick,yellow!60!black,every mark/.append style={solid,fill=yellow!80!black},mark=square*, only marks\\%
thick,purple,every mark/.append style={solid,fill=gray},mark=otimes*, only marks\\%
thick,blue,densely dashed,mark=star,every mark/.append style=solid, only marks\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*, only marks\\%
thick,colorbrewer4,mark=x\\%
thick,blue,every mark/.append style={fill=blue!80!black},mark=*\\%
}

\pgfplotscreateplotcyclelist{jianyucolor}{%
thin,black,mark=o,only marks\\%
thick,colorbrewer1,every mark/.append style={fill=colorbrewer1},mark=triangle*,only marks\\%
thick,orange,every mark/.append style={fill=orange},mark=square*,only marks\\%
thick, lime!80!black,every mark/.append style={fill=lime!80!black},mark=pentagon*,only marks\\%
thick,blue,every mark/.append style={fill=blue!80!black},mark=triangle*,only marks\\%
thick,cyan,every mark/.append style={fill=cyan},mark=square*,only marks\\%
thick,darkgreen,mark=pentagon*,only marks\\%
thick,yellow!60!black,every mark/.append style={solid,fill=yellow!80!black},mark=square*, only marks\\%
thick,purple,every mark/.append style={solid,fill=gray},mark=otimes*, only marks\\%
thick,blue,densely dashed,mark=star,every mark/.append style=solid, only marks\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*, only marks\\%
thick,colorbrewer4,mark=x\\%
thick,blue,every mark/.append style={fill=blue!80!black},mark=*\\%
red,every mark/.append style={fill=red!80!black},mark=square*\\%
brown!60!black,every mark/.append style={fill=brown!80!black},mark=diamond*\\%
blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*, only marks\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
brown!60!black,densely dashed,every mark/.append style={
solid,fill=brown!80!black},mark=square*\\%
darkred,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,densely dashed,mark=oplus,every mark/.append style=solid\\%
colorbrewer5,densely dashed,every mark/.append style={solid,fill=colorbrewer5},mark=diamond*\\%
darkgreen,densely dashed,mark=+,every mark/.append style=solid\\%
%red,blue,black,yellow,brown,teal,orange,violet\\%
thick,colorbrewer7,mark=triangle*\\%
thick,black,densely dashed\\%
thick,black\\%
}

\pgfplotscreateplotcyclelist{jianyucolorbar}{%
fill=black\\%
fill=colorbrewer1\\%
fill=orange\\%
fill=lime!80!black\\%
fill=blue\\%
fill=cyan\\%
fill=darkgreen\\%
fill=yellow!60!black\\%
thick,purple,every mark/.append style={solid,fill=gray}\\%
thick,blue,densely dashed,mark=star,every mark/.append style=solid\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*, only marks\\%
thick,colorbrewer4,mark=x\\%
thick,blue,every mark/.append style={fill=blue!80!black},mark=*\\%
red,every mark/.append style={fill=red!80!black},mark=square*\\%
brown!60!black,every mark/.append style={fill=brown!80!black},mark=diamond*\\%
blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*, only marks\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
brown!60!black,densely dashed,every mark/.append style={
solid,fill=brown!80!black},mark=square*\\%
darkred,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,densely dashed,mark=oplus,every mark/.append style=solid\\%
colorbrewer5,densely dashed,every mark/.append style={solid,fill=colorbrewer5},mark=diamond*\\%
darkgreen,densely dashed,mark=+,every mark/.append style=solid\\%
%red,blue,black,yellow,brown,teal,orange,violet\\%
thick,colorbrewer7,mark=triangle*\\%
thick,black,densely dashed\\%
thick,black\\%
}

\pgfplotscreateplotcyclelist{jianyucolorline}{%
thin,black\\%
thick,colorbrewer1,every mark/.append style={fill=colorbrewer1}\\%
thick,orange,every mark/.append style={fill=orange}\\%
thick, lime!80!black,every mark/.append style={fill=lime!80!black}\\%
thick,blue,every mark/.append style={fill=blue!80!black}\\%
thick,cyan,every mark/.append style={fill=cyan}\\%
thick,darkgreen\\%
thick,yellow!60!black,every mark/.append style={solid,fill=yellow!80!black}\\%
thick,purple,every mark/.append style={solid,fill=gray}\\%
thick,blue,densely dashed,mark=star,every mark/.append style=solid\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*, only marks\\%
thick,colorbrewer4,mark=x\\%
thick,blue,every mark/.append style={fill=blue!80!black},mark=*\\%
red,every mark/.append style={fill=red!80!black},mark=square*\\%
brown!60!black,every mark/.append style={fill=brown!80!black},mark=diamond*\\%
blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*, only marks\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
brown!60!black,densely dashed,every mark/.append style={
solid,fill=brown!80!black},mark=square*\\%
darkred,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,densely dashed,mark=oplus,every mark/.append style=solid\\%
colorbrewer5,densely dashed,every mark/.append style={solid,fill=colorbrewer5},mark=diamond*\\%
darkgreen,densely dashed,mark=+,every mark/.append style=solid\\%
%red,blue,black,yellow,brown,teal,orange,violet\\%
thick,colorbrewer7,mark=triangle*\\%
thick,black,densely dashed\\%
thick,black\\%
}

\pgfplotscreateplotcyclelist{jianyucolordistline}{%
thin,black,mark=*\\%
thin,colorbrewer1,every mark/.append style={fill=colorbrewer1},mark=triangle*\\%
thin,orange,every mark/.append style={fill=orange},mark=square*\\%
thin,lime!80!black,every mark/.append style={fill=lime!80!black},mark=pentagon*\\%
thin,blue,every mark/.append style={fill=blue!80!black},mark=triangle*\\%
thin,cyan,every mark/.append style={fill=cyan},mark=square*\\%
thin,darkgreen,mark=pentagon*\\%
densely dashed,black,mark=x\\%
thick,yellow!60!black,every mark/.append style={solid,fill=yellow!80!black}\\%
thick,purple,every mark/.append style={solid,fill=gray}\\%
thick,blue,densely dashed,mark=star,every mark/.append style=solid\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*, only marks\\%
thick,colorbrewer4,mark=x\\%
thick,blue,every mark/.append style={fill=blue!80!black},mark=*\\%
red,every mark/.append style={fill=red!80!black},mark=square*\\%
brown!60!black,every mark/.append style={fill=brown!80!black},mark=diamond*\\%
blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*, only marks\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
brown!60!black,densely dashed,every mark/.append style={
solid,fill=brown!80!black},mark=square*\\%
darkred,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,densely dashed,mark=oplus,every mark/.append style=solid\\%
colorbrewer5,densely dashed,every mark/.append style={solid,fill=colorbrewer5},mark=diamond*\\%
darkgreen,densely dashed,mark=+,every mark/.append style=solid\\%
%red,blue,black,yellow,brown,teal,orange,violet\\%
thick,colorbrewer7,mark=triangle*\\%
thick,black,densely dashed\\%
thick,black\\%
}

\pgfplotscreateplotcyclelist{jianyucolorboth}{%
thin,black,mark=o,only marks\\%
thick,colorbrewer1,every mark/.append style={fill=colorbrewer1},mark=triangle*,only marks\\%
thick,orange,every mark/.append style={fill=orange},mark=square*,only marks\\%
thick, lime!80!black,every mark/.append style={fill=lime!80!black},mark=pentagon*,only marks\\%
thick,blue,every mark/.append style={fill=blue!80!black},mark=triangle*,only marks\\%
thick,cyan,every mark/.append style={fill=cyan},mark=square*,only marks\\%
thick,darkgreen,mark=pentagon*,only marks\\% %%actual scattered points
thin,black\\%
thick,colorbrewer1,every mark/.append style={fill=colorbrewer1}\\%
thick,orange,every mark/.append style={fill=orange}\\%
thick, lime!80!black,every mark/.append style={fill=lime!80!black}\\%
thick,blue,every mark/.append style={fill=blue!80!black}\\%
thick,cyan,every mark/.append style={fill=cyan}\\%
thick,darkgreen\\% %%modeled lines
thick,yellow!60!black,every mark/.append style={solid,fill=yellow!80!black}\\%
thick,purple,every mark/.append style={solid,fill=gray}\\%
thick,blue,densely dashed,mark=star,every mark/.append style=solid\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*, only marks\\%
thick,colorbrewer4,mark=x\\%
thick,blue,every mark/.append style={fill=blue!80!black},mark=*\\%
red,every mark/.append style={fill=red!80!black},mark=square*\\%
brown!60!black,every mark/.append style={fill=brown!80!black},mark=diamond*\\%
blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*, only marks\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
brown!60!black,densely dashed,every mark/.append style={
solid,fill=brown!80!black},mark=square*\\%
darkred,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,densely dashed,mark=oplus,every mark/.append style=solid\\%
colorbrewer5,densely dashed,every mark/.append style={solid,fill=colorbrewer5},mark=diamond*\\%
darkgreen,densely dashed,mark=+,every mark/.append style=solid\\%
%red,blue,black,yellow,brown,teal,orange,violet\\%
thick,colorbrewer7,mark=triangle*\\%
thick,black,densely dashed\\%
thick,black\\%
}

\pgfplotscreateplotcyclelist{jianyu3color}{%
black,densely dashed\\%
black\\%
colorbrewer1,every mark/.append style={fill=colorbrewer1},mark=triangle*\\%
orange,every mark/.append style={fill=orange},mark=square*\\%
cyan,every mark/.append style={fill=cyan},mark=otimes*\\%
red!70!white,mark=star\\%
brown!60!black,every mark/.append style={fill=brown!80!black},mark=otimes*\\%
purple,every mark/.append style={solid,fill=gray},mark=otimes*\\%
very thick, blue,every mark/.append style={fill=lime},mark=diamond*\\%
very thick, darkgreen,mark=+,every mark/.append style=solid\\%
}

\pgfplotscreateplotcyclelist{jianyu4color}{%
black,densely dashed,mark=triangle*\\%
black,mark=triangle*\\%
colorbrewer1,densely dashed,mark=triangle*\\%
thick,colorbrewer1,mark=triangle*\\%
%colorbrewer1,densely dotted,mark=triangle*\\%
%colorbrewer1,densely dashdotted,mark=triangle*\\%
black,densely dashed,mark=square*\\%
black,mark=square*\\%
blue,densely dashed,mark=square*\\%
thick,blue,mark=square*\\%
%blue,densely dotted,mark=square*\\%
%blue,densely dashdotted,mark=square*\\%
black,densely dashed,mark=*\\%
black,mark=*\\%
darkgreen,densely dashed,mark=*\\%
thick,darkgreen,mark=*\\%
%darkgreen,densely dotted,mark=*\\%
%darkgreen,densely dashdotted,mark=*\\%
orange,mark=square\\%
cyan,mark=otimes\\%
purple,mark=star\\%
}


\pgfplotscreateplotcyclelist{jianyu5color}{%
black,densely dashed\\%
black\\%
darkgreen,densely dashed,mark=*\\%
thick,darkgreen,mark=*\\%
blue,densely dashed,mark=square*\\%
thick,blue,mark=square*\\%
colorbrewer1,densely dashed,mark=triangle*\\%
thick,colorbrewer1,mark=triangle*\\%
}

\pgfplotscreateplotcyclelist{jianyu6color}{%
black,densely dashed\\%
black\\%
very thick,densely dashed,colorbrewer1,every mark/.append style={fill=colorbrewer1},mark=triangle*\\%
very thick,orange,every mark/.append style={fill=orange},mark=square*\\%
cyan,every mark/.append style={fill=cyan},mark=otimes*\\%
red!70!white,mark=star\\%
brown!60!black,every mark/.append style={fill=brown!80!black},mark=otimes*\\%
purple,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,every mark/.append style={fill=lime},mark=diamond*\\%
darkgreen,mark=+,every mark/.append style=solid\\%
}


==> figures/find_model/preamble.tex <==
\usepackage{etex}

%\documentclass{sigplanconf}[10pt]
%\documentclass{sig-alternate}
%\documentclass{acm_proc_article-sp}
%\setlength{\textheight}{8.75in}
%\setlength{\textwidth}{6.5in}
%\setlength{\oddsidemargin}{0in}
%\setlength{\evensidemargin}{0in}
%\setlength{\topmargin}{-0.5in}

%\usepackage{amsmath}
\usepackage{comment}
\usepackage{tikz}
\usetikzlibrary{matrix,arrows,decorations.pathmorphing,patterns,positioning}
\usepackage{amssymb}
\usepackage{ifthen}
\usepackage{color}
\usepackage{colortbl}
\usepackage{rotating}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{url}
\usepackage{arydshln}

%\usepackage{pgfplots}
\usepackage{pgfplots}
%\pgfplotsset{compat=1.5}
%\pgfplotsset{compat=1.8}
%\usepgfplotslibrary{colorbrewer}

%\pgfplotsset{width=7cm,compat=1.13}

%\usetikzlibrary{external}
%\tikzexternalize[prefix=tikz/]

\usepackage{wrapfig}
%\usepackage{subfigure}
%\usepackage{subcaption}
\usepackage[font=small]{subcaption}
%\usepackage{caption}
%\usepackage[margin=0pt,labelsep=space,font=scriptsize,labelfont=bf,textfont=it,belowskip=-8pt,aboveskip=5pt]{caption}
%\usepackage[labelsep=space,font=small,aboveskip=5pt]{caption}
%\usepackage[font=small,labelfont=bf,textfont=normal,aboveskip=5pt]{caption}
\usepackage[font=small,labelfont=bf,textfont=it,aboveskip=5pt]{caption}
\usepackage{array}
\usepackage{framed}

\usepackage{balance}

\usepackage{epsfig}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
%\usepackage{algorithmicx}
%\usepackage{amsthm}

\usepackage{algorithmic}

%\usepackage[section]{algorithm}
\usepackage{algorithm}

\usepackage[normalem]{ulem}

%\usepackage{program}
\usepackage{ifthen}
\usepackage{boxedminipage}
\usepackage{fancyvrb}

\usepackage{soul}
\usepackage{graphicx}
\usepackage{graphics}
\usepackage{moreverb}
\usepackage{rotating}
\usepackage{enumerate}

\usepackage{enumitem}

\usepackage{tabularx,booktabs}

\usetikzlibrary{arrows}

%\usepackage{flushend}
\usepackage{xspace}

\usepackage{stmaryrd}



%\usepackage[absolute,showboxes]{textpos}
\usepackage[absolute]{textpos}
%set unit to be pagewidth and height, and increase inner margin of box
\setlength{\TPHorizModule}{\paperwidth}\setlength{\TPVertModule}{\paperheight}
\TPMargin{5pt}

\usepackage{listings}
\usepackage{xcolor}
\usepackage{fancyvrb}
\fvset{tabsize=2}
\definecolor{mygreen}{rgb}{0,0.6,0}
\lstset{ %
language=C,                % choose the language of the code
basicstyle=\footnotesize,       % the size of the fonts that are used for the code
commentstyle=\color{mygreen},
keywordstyle=\color{blue},
%numbers=left,                   % where to put the line-numbers
%numberstyle=\footnotesize,      % the size of the fonts that are used for the line-numbers
%stepnumber=1,                   % the step between two line-numbers. If it is 1 each line will be numbered
%numbersep=5pt,                  % how far the line-numbers are from the code
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
frame=single,           % adds a frame around the code
tabsize=1,          % sets default tabsize to 2 spaces
columns=fixed,
captionpos=b,           % sets the caption-position to bottom
breaklines=true,        % sets automatic line breaking
breakatwhitespace=true,    % sets if automatic breaks should only happen at whitespace
escapeinside={\%*}{*)}          % if you want to add a comment within your code
}            

%\pgfplotsset{every axis/.append style={
%        scaled y ticks = false, 
%        scaled x ticks = false, 
%        y tick label style={/pgf/number format/.cd, fixed, fixed zerofill,
%                            int detect,1000 sep={\;},precision=3},
%        x tick label style={/pgf/number format/.cd, fixed, fixed zerofill,
%                            int detect, 1000 sep={},precision=3}
%    }
%}

\special{papersize=8.5in,11in}
\setlength{\pdfpageheight}{\paperheight}
\setlength{\pdfpagewidth}{\paperwidth}

%\conferenceinfo{CONF 'yy}{Month d--d, 20yy, City, ST, Country} 
%\copyrightyear{20yy} 
%\copyrightdata{978-1-nnnn-nnnn-n/yy/mm} 
%\doi{nnnnnnn.nnnnnnn}

% Uncomment one of the following two, if you are not going for the 
% traditional copyright transfer agreement.

%\exclusivelicense                % ACM gets exclusive license to publish, 
                                  % you retain copyright

%\permissiontopublish             % ACM gets nonexclusive license to publish
                                  % (paid open-access papers, 
                                  % short abstracts)

%\titlebanner{banner above paper title}        % These are ignored unless
%\preprintfooter{short description of paper}   % 'preprint' option specified.


%\usepackage{lmodern}

\usepackage{afterpage}

%\usepackage{mathrsfs}
%% For \mathscr
\usepackage[mathscr]{eucal}

%bold math
\usepackage{bm}

\pgfplotscreateplotcyclelist{mycolorlist}{%
blue,every mark/.append style={fill=blue!80!black},mark=*\\%
red,every mark/.append style={fill=red!80!black},mark=square*\\%
brown!60!black,every mark/.append style={fill=brown!80!black},mark=otimes*\\%
black,mark=star\\%
blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
brown!60!black,densely dashed,every mark/.append style={
solid,fill=brown!80!black},mark=square*\\%
black,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,densely dashed,mark=star,every mark/.append style=solid\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*\\%
}



\definecolor{colorbrewer1}{RGB}{228,26,28}
\definecolor{colorbrewer2}{RGB}{55,126,184}
\definecolor{colorbrewer3}{RGB}{77,175,74}
\definecolor{colorbrewer4}{RGB}{152,78,163}
\definecolor{colorbrewer5}{RGB}{255,127,0}
%\definecolor{colorbrewer6}{RGB}{255,255,51}
\definecolor{colorbrewer7}{RGB}{166,86,40}
\definecolor{colorbrewer8}{RGB}{247,129,191}
\definecolor{colorbrewer9}{RGB}{153,153,153}

\definecolor{darkgreen}{rgb}{0,0.5,0}

\newcommand{\cblue}[1]{\textcolor{blue}{#1}}
\newcommand{\cgreen}[1]{\textcolor{darkgreen}{#1}}
\newcommand{\cpurple}[1]{\textcolor{purple}{#1}}
\newcommand{\cred}[1]{\textcolor{red}{#1}}

\definecolor{darkred}{rgb}{0.44,0,0}
\definecolor{darkgreen}{rgb}{0,0.44,0}
\definecolor{darkblue}{rgb}{0,0,0.44}
\definecolor{enrique}{rgb}{0,0,0}

\pgfplotscreateplotcyclelist{jianyu2color}{
	colorbrewer1, mark=*,\\
	colorbrewer2, mark=square*,\\
	colorbrewer3, mark=triangle*,\\
	colorbrewer4, mark=x,\\
	colorbrewer5, mark=*,\\
	%colorbrewer6, mark=square*, \\
	colorbrewer7, mark=triangle*,\\
	colorbrewer8, mark=+,\\
}

\pgfplotscreateplotcyclelist{jianyu0color}{%
thick,colorbrewer1,every mark/.append style={fill=colorbrewer1},mark=triangle*,only marks\\%
thick,orange,every mark/.append style={fill=orange},mark=square*,only marks\\%
thick, lime!80!black,every mark/.append style={fill=lime!80!black},mark=pentagon*,only marks\\%
%thick,red!70!white,mark=pentagon*,only marks\\%
thick,blue,every mark/.append style={fill=blue!80!black},mark=triangle*,only marks\\%
thick,cyan,every mark/.append style={fill=cyan},mark=square*,only marks\\%
thick,darkgreen,mark=pentagon*,only marks\\%
thick,yellow!60!black,every mark/.append style={solid,fill=yellow!80!black},mark=square*, only marks\\%
thick,purple,every mark/.append style={solid,fill=gray},mark=otimes*, only marks\\%
thick,blue,densely dashed,mark=star,every mark/.append style=solid, only marks\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*, only marks\\%
thick,colorbrewer4,mark=x\\%
thick,blue,every mark/.append style={fill=blue!80!black},mark=*\\%
}

\pgfplotscreateplotcyclelist{jianyucolor}{%
thin,black,mark=o,only marks\\%
thick,colorbrewer1,every mark/.append style={fill=colorbrewer1},mark=triangle*,only marks\\%
thick,orange,every mark/.append style={fill=orange},mark=square*,only marks\\%
thick, lime!80!black,every mark/.append style={fill=lime!80!black},mark=pentagon*,only marks\\%
thick,blue,every mark/.append style={fill=blue!80!black},mark=triangle*,only marks\\%
thick,cyan,every mark/.append style={fill=cyan},mark=square*,only marks\\%
thick,darkgreen,mark=pentagon*,only marks\\%
thick,yellow!60!black,every mark/.append style={solid,fill=yellow!80!black},mark=square*, only marks\\%
thick,purple,every mark/.append style={solid,fill=gray},mark=otimes*, only marks\\%
thick,blue,densely dashed,mark=star,every mark/.append style=solid, only marks\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*, only marks\\%
thick,colorbrewer4,mark=x\\%
thick,blue,every mark/.append style={fill=blue!80!black},mark=*\\%
red,every mark/.append style={fill=red!80!black},mark=square*\\%
brown!60!black,every mark/.append style={fill=brown!80!black},mark=diamond*\\%
blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*, only marks\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
brown!60!black,densely dashed,every mark/.append style={
solid,fill=brown!80!black},mark=square*\\%
darkred,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,densely dashed,mark=oplus,every mark/.append style=solid\\%
colorbrewer5,densely dashed,every mark/.append style={solid,fill=colorbrewer5},mark=diamond*\\%
darkgreen,densely dashed,mark=+,every mark/.append style=solid\\%
%red,blue,black,yellow,brown,teal,orange,violet\\%
thick,colorbrewer7,mark=triangle*\\%
thick,black,densely dashed\\%
thick,black\\%
}

\pgfplotscreateplotcyclelist{jianyucolorbar}{%
fill=black\\%
fill=colorbrewer1\\%
fill=orange\\%
fill=lime!80!black\\%
fill=blue\\%
fill=cyan\\%
fill=darkgreen\\%
fill=yellow!60!black\\%
thick,purple,every mark/.append style={solid,fill=gray}\\%
thick,blue,densely dashed,mark=star,every mark/.append style=solid\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*, only marks\\%
thick,colorbrewer4,mark=x\\%
thick,blue,every mark/.append style={fill=blue!80!black},mark=*\\%
red,every mark/.append style={fill=red!80!black},mark=square*\\%
brown!60!black,every mark/.append style={fill=brown!80!black},mark=diamond*\\%
blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*, only marks\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
brown!60!black,densely dashed,every mark/.append style={
solid,fill=brown!80!black},mark=square*\\%
darkred,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,densely dashed,mark=oplus,every mark/.append style=solid\\%
colorbrewer5,densely dashed,every mark/.append style={solid,fill=colorbrewer5},mark=diamond*\\%
darkgreen,densely dashed,mark=+,every mark/.append style=solid\\%
%red,blue,black,yellow,brown,teal,orange,violet\\%
thick,colorbrewer7,mark=triangle*\\%
thick,black,densely dashed\\%
thick,black\\%
}

\pgfplotscreateplotcyclelist{jianyucolorline}{%
thin,black\\%
thick,colorbrewer1,every mark/.append style={fill=colorbrewer1}\\%
thick,orange,every mark/.append style={fill=orange}\\%
thick, lime!80!black,every mark/.append style={fill=lime!80!black}\\%
thick,blue,every mark/.append style={fill=blue!80!black}\\%
thick,cyan,every mark/.append style={fill=cyan}\\%
thick,darkgreen\\%
thick,yellow!60!black,every mark/.append style={solid,fill=yellow!80!black}\\%
thick,purple,every mark/.append style={solid,fill=gray}\\%
thick,blue,densely dashed,mark=star,every mark/.append style=solid\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*, only marks\\%
thick,colorbrewer4,mark=x\\%
thick,blue,every mark/.append style={fill=blue!80!black},mark=*\\%
red,every mark/.append style={fill=red!80!black},mark=square*\\%
brown!60!black,every mark/.append style={fill=brown!80!black},mark=diamond*\\%
blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*, only marks\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
brown!60!black,densely dashed,every mark/.append style={
solid,fill=brown!80!black},mark=square*\\%
darkred,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,densely dashed,mark=oplus,every mark/.append style=solid\\%
colorbrewer5,densely dashed,every mark/.append style={solid,fill=colorbrewer5},mark=diamond*\\%
darkgreen,densely dashed,mark=+,every mark/.append style=solid\\%
%red,blue,black,yellow,brown,teal,orange,violet\\%
thick,colorbrewer7,mark=triangle*\\%
thick,black,densely dashed\\%
thick,black\\%
}

\pgfplotscreateplotcyclelist{jianyucolordistline}{%
thin,black,mark=*\\%
thin,colorbrewer1,every mark/.append style={fill=colorbrewer1},mark=triangle*\\%
thin,orange,every mark/.append style={fill=orange},mark=square*\\%
thin,lime!80!black,every mark/.append style={fill=lime!80!black},mark=pentagon*\\%
thin,blue,every mark/.append style={fill=blue!80!black},mark=triangle*\\%
thin,cyan,every mark/.append style={fill=cyan},mark=square*\\%
thin,darkgreen,mark=pentagon*\\%
densely dashed,black,mark=x\\%
thick,yellow!60!black,every mark/.append style={solid,fill=yellow!80!black}\\%
thick,purple,every mark/.append style={solid,fill=gray}\\%
thick,blue,densely dashed,mark=star,every mark/.append style=solid\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*, only marks\\%
thick,colorbrewer4,mark=x\\%
thick,blue,every mark/.append style={fill=blue!80!black},mark=*\\%
red,every mark/.append style={fill=red!80!black},mark=square*\\%
brown!60!black,every mark/.append style={fill=brown!80!black},mark=diamond*\\%
blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*, only marks\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
brown!60!black,densely dashed,every mark/.append style={
solid,fill=brown!80!black},mark=square*\\%
darkred,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,densely dashed,mark=oplus,every mark/.append style=solid\\%
colorbrewer5,densely dashed,every mark/.append style={solid,fill=colorbrewer5},mark=diamond*\\%
darkgreen,densely dashed,mark=+,every mark/.append style=solid\\%
%red,blue,black,yellow,brown,teal,orange,violet\\%
thick,colorbrewer7,mark=triangle*\\%
thick,black,densely dashed\\%
thick,black\\%
}

\pgfplotscreateplotcyclelist{jianyucolorboth}{%
thin,black,mark=o,only marks\\%
thick,colorbrewer1,every mark/.append style={fill=colorbrewer1},mark=triangle*,only marks\\%
thick,orange,every mark/.append style={fill=orange},mark=square*,only marks\\%
thick, lime!80!black,every mark/.append style={fill=lime!80!black},mark=pentagon*,only marks\\%
thick,blue,every mark/.append style={fill=blue!80!black},mark=triangle*,only marks\\%
thick,cyan,every mark/.append style={fill=cyan},mark=square*,only marks\\%
thick,darkgreen,mark=pentagon*,only marks\\% %%actual scattered points
thin,black\\%
thick,colorbrewer1,every mark/.append style={fill=colorbrewer1}\\%
thick,orange,every mark/.append style={fill=orange}\\%
thick, lime!80!black,every mark/.append style={fill=lime!80!black}\\%
thick,blue,every mark/.append style={fill=blue!80!black}\\%
thick,cyan,every mark/.append style={fill=cyan}\\%
thick,darkgreen\\% %%modeled lines
thick,yellow!60!black,every mark/.append style={solid,fill=yellow!80!black}\\%
thick,purple,every mark/.append style={solid,fill=gray}\\%
thick,blue,densely dashed,mark=star,every mark/.append style=solid\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*, only marks\\%
thick,colorbrewer4,mark=x\\%
thick,blue,every mark/.append style={fill=blue!80!black},mark=*\\%
red,every mark/.append style={fill=red!80!black},mark=square*\\%
brown!60!black,every mark/.append style={fill=brown!80!black},mark=diamond*\\%
blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
thick,red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*, only marks\\%
red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
brown!60!black,densely dashed,every mark/.append style={
solid,fill=brown!80!black},mark=square*\\%
darkred,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,densely dashed,mark=oplus,every mark/.append style=solid\\%
colorbrewer5,densely dashed,every mark/.append style={solid,fill=colorbrewer5},mark=diamond*\\%
darkgreen,densely dashed,mark=+,every mark/.append style=solid\\%
%red,blue,black,yellow,brown,teal,orange,violet\\%
thick,colorbrewer7,mark=triangle*\\%
thick,black,densely dashed\\%
thick,black\\%
}

\pgfplotscreateplotcyclelist{jianyu3color}{%
black,densely dashed\\%
black\\%
colorbrewer1,every mark/.append style={fill=colorbrewer1},mark=triangle*\\%
orange,every mark/.append style={fill=orange},mark=square*\\%
cyan,every mark/.append style={fill=cyan},mark=otimes*\\%
red!70!white,mark=star\\%
brown!60!black,every mark/.append style={fill=brown!80!black},mark=otimes*\\%
purple,every mark/.append style={solid,fill=gray},mark=otimes*\\%
very thick, blue,every mark/.append style={fill=lime},mark=diamond*\\%
very thick, darkgreen,mark=+,every mark/.append style=solid\\%
}

\pgfplotscreateplotcyclelist{jianyu4color}{%
black,densely dashed,mark=triangle*\\%
black,mark=triangle*\\%
colorbrewer1,densely dashed,mark=triangle*\\%
thick,colorbrewer1,mark=triangle*\\%
%colorbrewer1,densely dotted,mark=triangle*\\%
%colorbrewer1,densely dashdotted,mark=triangle*\\%
black,densely dashed,mark=square*\\%
black,mark=square*\\%
blue,densely dashed,mark=square*\\%
thick,blue,mark=square*\\%
%blue,densely dotted,mark=square*\\%
%blue,densely dashdotted,mark=square*\\%
black,densely dashed,mark=*\\%
black,mark=*\\%
darkgreen,densely dashed,mark=*\\%
thick,darkgreen,mark=*\\%
%darkgreen,densely dotted,mark=*\\%
%darkgreen,densely dashdotted,mark=*\\%
orange,mark=square\\%
cyan,mark=otimes\\%
purple,mark=star\\%
}


\pgfplotscreateplotcyclelist{jianyu5color}{%
black,densely dashed\\%
black\\%
darkgreen,densely dashed,mark=*\\%
thick,darkgreen,mark=*\\%
blue,densely dashed,mark=square*\\%
thick,blue,mark=square*\\%
colorbrewer1,densely dashed,mark=triangle*\\%
thick,colorbrewer1,mark=triangle*\\%
}

\pgfplotscreateplotcyclelist{jianyu6color}{%
black,densely dashed\\%
black\\%
very thick,densely dashed,colorbrewer1,every mark/.append style={fill=colorbrewer1},mark=triangle*\\%
very thick,orange,every mark/.append style={fill=orange},mark=square*\\%
cyan,every mark/.append style={fill=cyan},mark=otimes*\\%
red!70!white,mark=star\\%
brown!60!black,every mark/.append style={fill=brown!80!black},mark=otimes*\\%
purple,every mark/.append style={solid,fill=gray},mark=otimes*\\%
blue,every mark/.append style={fill=lime},mark=diamond*\\%
darkgreen,mark=+,every mark/.append style=solid\\%
}


==> limitations.tex <==
1. require large $ k $ ( $ k > 512 $ ).


==> method.tex <==
%2. Build a performance model for Tensor Contraction (which modification do we need to add considering those scatter/gather instructions?)
%3. Code generation for the scatter/gather micro-kernel (Not sure if we need this yet.)
%4. Evaluate the performance for various platforms, e.g. Intel Ivy Bridge, ARM v8, KNL, etc.

\input tensor






